Personalized Federated Learning with Moreau Envelopes

Federated learning (FL) is a decentralized and privacy-preserving machine learning technique in which a group of clients collaborate with a server to learn a global model without sharing clients' data. One challenge associated with FL is statistical diversity among clients, which restricts the global model from delivering good performance on each client's task. To address this, we propose an algorithm for personalized FL (pFedMe) using Moreau envelopes as clients' regularized loss functions, which help decouple personalized model optimization from the global model learning in a bi-level problem stylized for personalized FL. Theoretically, we show that pFedMe's convergence rate is state-of-the-art: achieving quadratic speedup for strongly convex and sublinear speedup of order 2/3 for smooth nonconvex objectives. Experimentally, we verify that pFedMe excels at empirical performance compared with the vanilla FedAvg and Per-FedAvg, a meta-learning based personalized FL algorithm.

==> experiments.tex <==
In this section, we validate the performance of \OurAlg when the data distributions are heterogeneous and non-i.i.d. We  compare \OurAlg with FedAvg and Per-FedAvg in both $\mu$-strongly convex and nonconvex settings. The effect of hyperparameters is presented in the supplementary document. %The experimental results show that our algorithm gains noticeable performance improvement from the vanilla FedAvg and  Per-FedAvg in terms of training loss convergence rate and test accuracy in various settings.

\subsection{Experimental Settings}
%The goals in this section are:
%\begin{itemize}
%	\item to identify the effect of hyperparameters such as $R$, $K$ and $\lambda$ to the convergence and performance of our algorithm;
%	\item to compare the performance, in terms of train loss and global accuracy, of our algorithm with those of FedAvg, Per-FedAvg and APFL; and
%	\item to compare the performances, in terms of test accuracy, of the algorithms above when using their best combination of hyperparameters.
%\end{itemize}
We consider a classification problem using both  real  (MNIST) and  synthetic datasets. MNIST \cite{lecun_gradient-based_1998} is a handwritten digit dataset containing 10 labels and 70,000 instances. Due to the limitation on MNIST's data size, we distribute the complete dataset to $ N = 20$ clients. To model a heterogeneous setting in terms of local data sizes and classes,  each client is allocated a different local data size in the range of $[1165, 3834]$, and only has 2 of the 10 labels. For synthetic data, we adopt the data generation and distribution procedure from \cite{li_federated_2019}, using two parameters $\bar{\alpha}$ and $\bar{\beta}$ to control how much the local model and the dataset of each client differ, respectively. Specifically, the dataset serves a 10-class classifier using 60-dimensional real-valued data. We generate a synthetic dataset with $\bar{\alpha} = 0.5$ and $\bar{\beta} =0.5$.  Each client's data size is in the range of $[250, 25810]$. Finally, we distribute the data to $ N = 100$ clients according to the power law in \cite{li_federated_2019}. 

We fix the subset of clients %$|\mathcal{D}_{i, r}^t| = 20$ for all datasets and set 
$S = 5$ for MNIST, and $S = 10$ for Synthetic.  We compare the algorithms using both cases of the same and fine-tuned learning rates, batch sizes, and number of local  and global iterations. For $\mu$-strongly convex setting, we consider a $l_2$-regularized multinomial logistic regression model (MLR) with the softmax activation and cross-entropy loss functions. 
%The $\mu$-strongly convex loss function $f_i(\theta)$ is defined as follows:
%\begin{align*}
%f_i(\theta) = -\frac{1}{M}\biggS{\sum_{m=1}^{M}\sum_{c=1}^{C}1\{y^{(m)} = c\} log\frac{exp(\theta^{(c)T}x^m)}{\sum_{j=1}^{C}exp(\theta^{(j)T}x^m)}} + \frac{\mu}{2} |\theta|^2
%\end{align*}
For nonconvex case, a two-layer deep neural network (DNN) is implemented with hidden layer of size $100$ for MNIST and $20$ for Synthetic using ReLU activation and a softmax layer at the end. In \OurAlg, we use gradient descent to obtain $\delta$-approximate $\tilde{\theta}_i (w_{i, r}^t)$ and the personalized model is evaluated on the personalized parameter $\tilde\theta_i$ while the global model is evaluated on $w$. For the comparison with Per-FedAvg, we use its personalized model which is the local model after taking an SGD step from the global model. All datasets are split randomly with 75\% and 25\% for training and testing, respectively. %For Per-FedAvg, a one-step update is used during validation on the test set.  so the test data and train data over the nodes have the same distribution.
%. For each comparison, we fix the randomly selected devices, the stragglers, and mini-batch orders across all runs.
%As a note during the evaluation, we use both the global model ($w^t_i$) and the personalized model ($\theta^t_i$) to indicate their difference, especially the performance gain when using the personalized model.
All experiments were conducted using PyTorch \cite{paszke_pytorch_2019} version 1.4.0. 
%The code and datasets are available online\footnote{\href{https://github.com/CharlieDinh/pFedMe}{https://github.com/CharlieDinh/pFedMe}}.

%\subsection{Effect of hyperparameters on Personalized Federated Learning's convergence}

%% -------- Logistic -----------
%%\begin{figure*}
%%	\begin{multicols}{3}
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_fixR.pdf}\par
%%		\captionof{figure}{Effect of $K$ Convex}
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_fixK.pdf}\par
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_fixL.pdf}\par
%%	\end{multicols}
%%	\begin{multicols}{3}
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_fixR.pdf}\par
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_fixK.pdf}\par
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_fixL.pdf}\par
%%	\end{multicols}
%%	\caption{caption here}
%%\end{figure*}
%%\begin{figure}[t!]
%%	\begin{subfigure}{0.31\linewidth} % width of right subfigure
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_fixR.pdf}
%%		\caption{Effect of $R$ (Convex)} %on both the global model and the personalized mode
%%		\label{F:ConR}
%%	\end{subfigure}
%%	\begin{subfigure}{0.31\linewidth} % width of right subfigure
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_fixK.pdf}
%%		\caption{Effect of $K$  (Convex)} %on both the global model and the personalized mode
%%		\label{F:ConK}
%%	\end{subfigure}
%%	\begin{subfigure}{0.31\linewidth} % width of right subfigure
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_fixL.pdf}
%%		\caption{Effect of $\lambda$  (Convex)} %on both the global model and the personalized mode
%%		\label{F:ConL}
%%	\end{subfigure}\\
%%	\begin{subfigure}{0.31\linewidth} % width of right subfigure
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_fixR.pdf}
%%		\caption{Effect of $R$  (Non Convex)} %on both the global model and the personalized mode
%%		\label{F:NonConR}
%%	\end{subfigure}
%%	\begin{subfigure}{0.31\linewidth} % width of right subfigure
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_fixK.pdf}
%%		\caption{Effect of $K$  (Non Convex)} %on both the global model and the personalized mode
%%		\label{F:NonConK}
%%	\end{subfigure}
%%	\begin{subfigure}{0.31\linewidth} % width of right subfigure
%%		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_fixL.pdf}
%%		\caption{Effect of $\lambda$  (Non Convex)} %on both the global model and the personalized mode
%%		\label{F:NonConL}
%%	\end{subfigure}
%%	\caption{Effect of $\lambda$, $K$ steps, and $R$ local rounds on Personalized Federated Learning convergence in both the convex and non convex setting ($\eta=0.005$, $|\mathcal{D}_{i, r}^t| = 20$, $N = 10$ for all experiments) }. %In Fig.~\ref{F:R} , Fig.~\ref{F:K} , Fig.~\ref{F:lambda}}
%%	\label{F:Log}
%%\end{figure}
%
%
%
%%
%%\begin{figure}
%%	\centering
%%	\includegraphics[width=0.8\linewidth]{Image/Mnist/MNIST-algorithm-comparison-nonconvex.pdf}
%%	\caption{Performance comparison of Personalized FedAvg (global and personalized models), FedAvg and Per-FedAvg in the nonconvex setting using the MNIST dataset. $\eta=0.003$, $|\mathcal{D}_{i, r}^t| = 20$, $N = 5$, $\lambda = 15$}
%%	\label{F:Mnist_convex}
%%\end{figure}
%
%%\begin{figure}
%%	\centering
%%	\includegraphics[width=0.8\linewidth]{Image/Mnist/MNIST-algorithm-comparison-convex.pdf}
%%	\caption{Performance comparison of Personalized FedAvg (global and personalized models), FedAvg and Per-FedAvg in the convex setting using the MNIST dataset. $\eta=0.003$, $|\mathcal{D}_{i, r}^t| = 20$, $N = 5$, $\lambda = 15$}
%%	\label{F:Mnist_nonconvex}
%%\end{figure}
%
%
%To understand how different values of hyperparameters $R$, $K$, $|\mathcal{D}|$, $\lambda$, and $\beta$  affect the convergence of \OurAlg in both $\mu$-strongly convex and nonconvex settings, we conduct various experiments on MNIST dataset.% shown on Fig.~\ref{F:Log}.
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_R.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_R.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy1}
%	\end{subfigure}
%	%	\hspace{1em} % here you can insert horizontal or vertical space
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_R.pdf}
%		%\caption{$\mu$-strongly convex seting (MNIST)}
%		\label{F:Mnist_loss1}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_R.pdf}
%		%\caption{Non-convex  seting (MNIST)}
%		\label{F:Mnist_loss2}
%	\end{subfigure}
%	\caption{Effect of $R$ on convergence of \OurAlg in $\mu$-strongly convex and nonconvex setting on MNIST.}
%	\label{F:Mnist_R}
%\end{figure}
%
%\textbf{Effects of local computation rounds $R$}:
%When communication is relatively costly, the server tends to allow users to have more local computation. This can lead to further update to the global model after each round of communication, allowing it to converge faster. Therefore, we monitor the behavior of \OurAlg using a number of values of $R$, which results in Fig.~\ref{F:Mnist_R} for $\mu$-strongly convex setting and the nonconvex setting, respectively. The results show that the larger values of $R$ have a benefit on the convergence of both the personalized and the global models.  There is, nevertheless, a trade-off between computation and communication: while larger $R$ requires more computation at local users, smaller $R$ needs more global communication rounds to converge. To balance this trade-off, we fix $R = 20$ and evaluate the effect of other hyperparameters accordingly.
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_K.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_K.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy1}
%	\end{subfigure}
%	%	\hspace{1em} % here you can insert horizontal or vertical space
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_K.pdf}
%		%\caption{$\mu$-strongly convex seting (MNIST)}
%		\label{F:Mnist_loss1}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_K.pdf}
%		%\caption{Non-convex  seting (MNIST)}
%		\label{F:Mnist_loss2}
%	\end{subfigure}
%	\caption{Effect of $K$ steps on convergence of \OurAlg in $\mu$-strongly convex and non convex settings on MNIST.} 
%	\label{F:Mnist_K}
%\end{figure}
%
%\textbf{Effects of number steps $K$}: As $K$ allows calculating approximate the personalized model $\theta$, $K$ is also considered as a hyper-parameter of \OurAlg. In Fig.~\ref{F:Mnist_K}, only the value of $K$ is changed during the experiments. We observe that \OurAlg requires a small value of $K$ around 3, 5 steps to approximately compute the personalized model. The larger $K$ for example 7, does not improve much on the convergence of the personalized model and the global as well. Similar to $R$, the larger $K$ also requires more user's computation, which has negative effects on user energy consumption. Therefore, the value of $K = 5$ is chosen for remaining experiments.
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_D.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_D.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy1}
%	\end{subfigure}
%	%	\hspace{1em} % here you can insert horizontal or vertical space
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_D.pdf}
%		%\caption{$\mu$-strongly convex seting (MNIST)}
%		\label{F:Mnist_loss1}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_D.pdf}
%		%\caption{Non-convex  seting (MNIST)}
%		\label{F:Mnist_loss2}
%	\end{subfigure}
%	\caption{Effect of $|\mathcal{D}|$ on convergence of \OurAlg in $\mu$-strongly  convex and nonconvex settings on MNIST.} 
%	\label{F:Mnist_D}
%\end{figure}
%
%\textbf{Effects of Mini-Batch size $|\mathcal{D}|$}: As mentioned in the Lamda \ref{lem:1}, $| \mathcal {D} | $ is one of the parameters which can be controlled to adjust the value of $\delta$. In Fig.~\ref{F:Mnist_D}, when the size of the mini-batch is increased, \OurAlg has a higher convergence rate. However, the too-large of $| \mathcal {D}| $ will not only slow the convergence of \OurAlg but also requires higher computation at the local users. During the experiments, the value of $ | \mathcal {D}| $ is configured as a constant value equal to 20.
%
%%One of the most important factors 
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_L.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_L.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy1}
%	\end{subfigure}
%	%	\hspace{1em} % here you can insert horizontal or vertical space
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_L.pdf}
%		%\caption{$\mu$-strongly convex seting (MNIST)}
%		\label{F:Mnist_loss1}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_L.pdf}
%		%%\caption{Non-convex  seting (MNIST)}
%		\label{F:Mnist_loss2}
%	\end{subfigure}
%	\caption{Effect of $\lambda$ on convergence of \OurAlg in $\mu$-strongly convex and nonconvex settings on MNIST. }
%	\label{F:Mnist_L}
%\end{figure}
%\textbf{Effects of regularization $\lambda$}: Fig.~\ref{F:Mnist_L} shows the convergence rate of \OurAlg with different values of $\lambda$ in the $\mu$-strongly convex setting and the nonconvex setting. As can be seen, in all settings, the larger $\lambda$ allows faster convergence; however, we also observe that the significant large $\lambda$ will hurt the performance of \OurAlg by making \OurAlg divergence. This result fits perfectly with our convergence analysis. %on Theo %since proximal regularization parameter $\lambda$  $\delta$ can be adjusted by controlling the (i)  sampling error using mini-batch size $\abs{\mathcal{D}^{i}}$, (ii) accuracy level $\nu$, and (iii) proximal regularization parameter $\lambda$. . %More interestingly, \OurAlg gains significant convergence improvement in both personalized model and global model (with sufficient $\lambda$, and $K$) compared to other algorithms even in the convex setting or the nonconvex setting.

%\textbf{Effects of $\beta$}:
%Fig.~\ref{F:Mnist_Beta} illustrates how moving averaging parameter $\beta$ ($\beta \geq 1$) affects both the personalized model and the global model. It is noted that when $\beta = 1$, it is similar to model averaging of FedAvg. According to the figure, it is beneficial to shift the value of $\beta$ to be larger as it allows the global and the personalized model to converge faster. Besides, turning $\beta$ carefully is also significant to prevent the divergence and instability of \OurAlg. For example, when $\beta$ moves to the large value of 5, even though the personalized model has higher testing accuracy and smaller training loss, the global model starts to fluctuate and if $\beta > 5$, the global model will become unsteady. Consequently, in this experiment, $\beta =2$ can be considered as an optimized value to reach the balance between the global model and the personalized model.%In this %We examine the several values of $\beta
%Fig.~\ref{F:Mnist_Beta} illustrates how moving averaging parameter $\beta$ ($\beta \geq 1$) affects both the personalized model and the global model. It is noted that when $\beta = 1$, it is similar to model averaging of FedAvg. According to the figure, it is beneficial to shift the value of $\beta$ to be larger as it allows \OurAlg to converge faster, especially the global model. However, turning $\beta$ carefully is also significant to prevent the divergence and instability of \OurAlg. For example, when $\beta$ moves to the large value, to stable the global model as well as the personalized model, the smaller value of $\eta$ needs to be considered. Alternatively, $\beta$  and $\eta$ should be adjusted in inverse proportion to reach the stability of \OurAlg.
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_Beta.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of left subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_Beta.pdf}
%		%\caption{Average testing accurancy }
%		\label{F:Mnist_accurancy1}
%	\end{subfigure}
%	%	\hspace{1em} % here you can insert horizontal or vertical space
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_Beta.pdf}
%		\label{F:Mnist_loss1}
%	\end{subfigure}
%	\begin{subfigure}{0.245\linewidth} % width of right subfigure
%		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_Beta.pdf}
%		\label{F:Mnist_loss2}
%	\end{subfigure}
%	\caption{Effect of $\beta$ on convergence of \OurAlg in $\mu$-strongly convex and nonconvex settings on MNIST. }
%	\label{F:Mnist_Beta}
%\end{figure}
\subsection{Effect of hyperparameters}
To understand how different hyperparameters such as $K$ and $\beta$  affect the convergence of \OurAlg in both $\mu$-strongly convex and nonconvex settings, we conduct various experiments on MNIST dataset with $\eta = 0.005$ and $S = 5$. The explanations for choosing the range of hyperparameters  $R$, $|\mathcal{D}|$, and $\lambda$ are provided in the supplementary files.

\textbf{Effects of computation complexity $K$}: As $K$ allows for approximately finding the personalized model $\theta$, $K$ is also considered as a hyper-parameter of \OurAlg. In Fig.~\ref{F:Mnist_K}, only the value of $K$ is changed during the experiments. We observe that \OurAlg requires a small value of $K$ (around 3 to 5 steps) to approximately compute the personalized model. Larger values of $K$, such as 7, do not show the improvement on the convergence of the personalized model nor the global model. Similar to $R$, larger $K$ also requires more user's computation, which has negative effects on user energy consumption. Therefore, the value of $K = 5$ is chosen for the remaining experiments.

\begin{figure}[t!]
	\centering
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_K.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_K.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy1}
	\end{subfigure}
	% \hspace{1em} % here you can insert horizontal or vertical space
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_K.pdf}
		%\caption{$\mu$-strongly convex seting (MNIST)}
		\label{F:Mnist_loss1}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_K.pdf}
		%\caption{nonconvex  seting (MNIST)}
		\label{F:Mnist_loss2}
	\end{subfigure}
	\caption{Effect of $K$ on the convergence of \OurAlg in $\mu$-strongly convex and nonconvex settings on MNIST ($|\mathcal{D}| = 20$, $\lambda = 15$, $R = 20$, $\beta =1$).} 
	\label{F:Mnist_K}
\end{figure}


%\textbf{Effects of regularization $\lambda$}: Fig.~\ref{F:Mnist_L} shows the convergence rate of \OurAlg with different values of $\lambda$. In all settings, larger $\lambda$ allows for faster convergence; however, we also observe that the significantly large $\lambda$ will hurt the performance of \OurAlg by making \OurAlg diverge. Therefore, $\lambda$ should be tuned carefully depending on the dataset. We fix $\lambda= 15$ for all scenarios with MNIST.

\textbf{Effects of $\beta$}:
Fig.~\ref{F:Mnist_Beta} illustrates how $\beta$ ($\beta \geq 1$) affects both the personalized and global models. It is noted that when $\beta = 1$, it is similar to model averaging of FedAvg. According to the figure, it is beneficial to shift the value of $\beta$ to be larger as it allows \OurAlg to converge faster, especially the global model. However, turning $\beta$ carefully is also significant to prevent the divergence and instability of \OurAlg. For example, when $\beta$ moves to the large value, to stabilize the global model as well as the personalized model, the smaller value of $\eta$ needs to be considered. Alternatively, $\beta$  and $\eta$ should be adjusted in inverse proportion to reach the stability of \OurAlg.
\begin{figure}[t!]
	\centering
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_Beta.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_Beta.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy1}
	\end{subfigure}
	% \hspace{1em} % here you can insert horizontal or vertical space
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_Beta.pdf}
		\label{F:Mnist_loss1}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_Beta.pdf}
		\label{F:Mnist_loss2}
	\end{subfigure}
	\caption{Effect of $\beta$ on the convergence of \OurAlg in $\mu$-strongly convex and nonconvex settings on MNIST ($|\mathcal{D}| = 20$, $\lambda = 15$, $R = 20$, $K = 5$).}
	\label{F:Mnist_Beta}
\end{figure}

\subsection{Performance Comparison}
In order to highlight the empirical performance of \OurAlg,  we perform several comparisons between \OurAlg, FedAvg, and Per-FedAvg. We first use the same parameters for all algorithms as an initial comparison. As algorithms behave differently when hyperparameters are changed, we conduct a grid search on a wide range of hyperparameters to figure out the combination of fine-tuned parameters that achieves the highest test accuracy w.r.t. each algorithm. We use both personalized model (PM) and the global model (GM) of \OurAlg for comparisons. 

%\begin{table}[t!]
%	\centering
%	\caption{Comparision using optimized hyperparameters for Synthetic. We fix $|\mathcal{D}| = 20$, $R = 20$, $K =5$, and $T = 600$ ($\hat{\alpha}$ and $\hat{\beta}$ are learning rates of Per-FedAvg).}
%	\label{Tab:parameters2}
%	\begin{tabular}{llllll}
%		\cmidrule(r){1-6}
%		Algorithms & Dataset & Model & $\lambda$ & $\eta$   & $Acc$\\
%		\midrule
%		FedAvg  & Synthetic& Logistic & $$  & $0.02$   & $77.86\% $\\
%		Per-FedAvg & Synthetic& Logistic & $$   & $0.01$($\hat{\alpha}$)/$0.001$($\hat{\beta})$   & $79.91\% $\\
%		\OurAlg-Global Model& Synthetic & Logistic & $20$  &  $0.01$   & $79.28 \% $\\
%		\OurAlg-Personal Model & Synthetic& Logistic& $20$  &  $0.01$  & $82.55 \% $\\
%		\midrule
%		FedAvg  & Synthetic& DNN & $$  & $0.03$   & $83.32\% $\\
%		Per-FedAvg & Synthetic& DNN & $$   & $0.01$($\hat{\alpha}$)/$0.001$($\hat{\beta})$  & $84.76\% $\\
%		\OurAlg-Global Model & Synthetic& DNN & $20$  &  $0.01$   & $84.44 \% $\\
%		\OurAlg-Personal Model & Synthetic& DNN& $20$  &  $0.01$  & $85.08 \% $\\
%		\bottomrule
%	\end{tabular}
%\end{table}
%\begin{table}[h!]
%	\centering
%	\begin{tabular}{| c | c | c | c | c | c | c | c | c |} 
%		\hline
%		Dataset & $\lambda$  & $K$ & $B$ & $\eta$  & $R$ & $T$   & $Accurancy$\\
%		\hline
%		Fedavg  & $$ & $$ & 20& $0.005$ & $20$ & $1000$  & $94.00\% $\\
%		Per-FedAvg & $$  & $$ & 20 & $0.005(\alpha)/0.001(\beta)$ & $20$ & $1000$  & $92.50\% $\\
%		Our Agorithm-Persional Model & $3$ & $5$ & 20& $0.005$ & $20$ & $1000$  & $92.00 \% $\\
%		Our Agorithm-Global Model & $3$ & $5$ & 20& $0.005$ & $20$ & $1000$  & $92.00 \% $\\
%		\hline
%	\end{tabular}
%
%	\caption{Experiment  parameters. ($\alpha$ and $\beta$ are learning rates of Per-FedAvg) } \label{T:parameters}
%\end{table}

%Regarding the results on the MNIST dataset in Fig.~\ref{F:Mnist} and Table.~\ref{Tab:parameters1}, even if the fine-tuned parameters or similar parameters are selected, \OurAlg outperforms others in terms of training loss and testing accuracy for both the personalized model and the global model with respect to the $\mu$-strongly convex setting. Only in the nonconvex setting, there is marginally different. When using the same parameters, the global model of \OurAlg converges faster than FedAvg and slightly slower than Per-Fedavg, while the personalized model of \OurAlg still gains a significant gap compared to others using the same parameter. In the case \blue{of fine-tuned parameters, \OurAlg outperforms others with respect to the personalized model and the global model}. 
\begin{figure}[t!]
	\centering
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_test_Com.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_test_Com.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy1}
	\end{subfigure}
	%	\hspace{1em} % here you can insert horizontal or vertical space
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTConvex_Mnist_train_Com.pdf}
		%\caption{$\mu$-strongly convex  seting}
		\label{F:Mnist_loss1}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Mnist/MNISTNon_Convex_Mnist_train_Com.pdf}
		%%\caption{Non-convex  seting}
		\label{F:Mnist_loss2}
	\end{subfigure}
	\caption{Performance comparison of \OurAlg, FedAvg, and Per-FedAvg in $\mu$-strongly convex and nonconvex settings using MNIST  ($\eta=0.005$, $|\mathcal{D}| = 20$, $S = 5$, $\beta =1$ for all experiments).}
	\label{F:Mnist}
\end{figure}

\begin{figure}[t!]
	\centering
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_test_Com.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of left subfigure
		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_test_Com.pdf}
		%\caption{Average testing accurancy }
		\label{F:Mnist_accurancy1}
	\end{subfigure}
	%	\hspace{1em} % here you can insert horizontal or vertical space
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICConvex_Syn_train_Com.pdf}
		%\caption{$\mu$-strongly convex seting}
		\label{F:Mnist_loss1}
	\end{subfigure}
	\begin{subfigure}{0.245\linewidth} % width of right subfigure
		\includegraphics[width=1\linewidth]{Image/Synthetic/LOGISTIC_SYNTHETICNon_Convex_Syn_train_Com.pdf}
		%%\caption{Non-convex  seting}
		\label{F:Mnist_loss2}
	\end{subfigure}
	\caption{Performance comparison of \OurAlg, FedAvg, and Per-FedAvg in $\mu$-strongly convex and nonconvex settings using Synthetic ($\eta=0.005$, $|\mathcal{D}| = 20$, $S = 10$, $\beta =1$ for all experiments).} %\blue{The accuracy improvements for the personalized model in the strongly convex setting are 5.4\%, 3.6\%, and 4.8\% compared to the global model, Per-FedAvg, and FedAvg respectively. The corresponding figures for the nonconvex setting are 3.7\%, 0.9\%, and 2.7\%.} }%\blue{ In the strongly convex case, the personalized model of \OurAlg achieves the highest accuracy at 95.30\%, following by the global model at 94,29\%, Per-Avg at 93.95\%, and FedAvg at 93,71. In the nonconvex case, the personalized model of \OurAlg achieves the highest accuracy at 98.41\%, following by Per-FedAvg at 97,64\%,  the global model at 97.68\%, and FedAvg at 97,24\%.} .}
	\label{F:Synthetic}
\end{figure}


The comparisons for MNIST dataset are shown in Fig.~\ref{F:Mnist} (the same hyperparameters) and Table.~\ref{Tab:parameters1} (fine-tuned hyperparameters). Fig.~\ref{F:Mnist} shows that the \OurAlg's personalized models in strongly convex setting are 1.1\%, 1.3\%, and 1.5\% more accurate than its global model, Per-FedAvg, and FedAvg, respectively. The corresponding figures for  nonconvex setting are 0.9\%, 0.9\%, and 1.3\%. Table.~\ref{Tab:parameters1} shows that when using fine-tuned hyperparameters, the \OurAlg's personalized model is the best performer in all settings.

%In $\mu$-strongly convex setting, even if the fine-tuned parameters or similar parameters are selected, \OurAlg outperforms others in terms of training loss and testing accuracy for both the personalized model and the global model. Only in the nonconvex setting, there is marginally different. When using the same parameters, the global model of \OurAlg converges faster than FedAvg and slightly slower than Per-Fedavg, while the personalized model of \OurAlg still gains a significant gap compared to others using the same parameter. In the case \blue{of fine-tuned parameters, \OurAlg outperforms others with respect to the personalized model and the global model}. 

For Synthetic dataset, the comparisons for the utilizing the same parameters and the fine-tuned parameter are presented in Fig.~\ref{F:Synthetic} and Table.~\ref{Tab:parameters1}, respectively. In  Fig.~\ref{F:Synthetic}, even though the global model of \OurAlg is less well-performed than others concerning testing accuracy and training loss, \OurAlg's personalized model still shows its advantages as achieving the highest testing accuracy and smallest training loss. Fig.~\ref{F:Synthetic} shows that \OurAlg's personalized model is  6.1\%, 3.8\%, and 5.2\% more accurate than its global model, Per-FedAvg, and FedAvg, respectively. The corresponding figures for the nonconvex setting are 3.9\%, 0.7\%, and 3.1\%. In addition, with fine-tuned hyperparameters in Table.~\ref{Tab:parameters1}, the personalized model of \OurAlg beats others in all settings while the global model of \OurAlg only performs better than FedAvg. % witness a similar trend in terms of the personalized model. %Only the personal model does not perform as good as Per-Avg and FedAvg.
% -------- MNIST-----------

{%\small
\begin{table}[t!]
	\centering
	\caption{Comparison {using fine-tuned hyperparameters}. We fix $|\mathcal{D}| = 20$, $R = 20$, $K =5$, and $T = 800$ for MNIST, and $T = 600$ for Synthetic, $\beta = 2$ for \OurAlg ($\hat{\alpha}$ and $\hat{\beta}$ are learning rates of Per-FedAvg).}
	\label{Tab:parameters1}
	\tabcolsep=0.11cm
		\begin{tabular}{ll|lll|lll}
		\cmidrule(lr){1-8}
		%\hline
		\multirow{2}{*}{Algorithm} &
		\multirow{2}{*}{Model} &
		%\multicolumn{6}{c}{Dataset} \\
		%\cmidrule(lr){3-8} & &
		 \multicolumn{3}{c}{MNIST} & \multicolumn{3}{|c}{Synthetic} \\
		\cmidrule(lr){3-5}\cmidrule(lr){6-8}
		%\cline{3-8}
		&  & $\lambda$ & $\eta \, (\hat{\alpha}, \hat{\beta})$    & $\text{  Accuracy (\%)}$ &$\lambda$ & $\eta \, (\hat{\alpha}, \hat{\beta})$      & $\text{  Accuracy (\%)}$ \\
%			&  & $\lambda$ & $\eta \, (\hat{\alpha}, \hat{\beta} \text{ \small for Per-FedAvg})$    & $\text{ \small Accuracy (\%)}$ &$\lambda$ & $\eta \, (\hat{\alpha}, \hat{\beta} \text{ \small for Per-FedAvg})$    & $\text{ \small Accuracy (\%)}$ \\
		\cmidrule(lr){1-8}
		FedAvg & MLR & & $0.02$  & $93.96 \pm 0.02 $& & $0.02$  & $77.62 \pm 0.11 $\\
		Per-FedAvg & MLR& & $0.03, 0.003$   & $94.37 \pm 0.04$& & $0.02, 0.002$ & $81.49 \pm 0.09 $\\
		\OurAlg-GM & MLR& 15& $0.01$& $ 94.18 \pm 0.06$ & 20 & $0.01$ & $78.65  \pm 0.25$ \\
		\OurAlg-PM & MLR& 15& $0.01$& $\textbf{95.62}\pm 0.04$ & 20 & $0.01$ & $\textbf{83.20}\pm 0.06 $ \\
		\cmidrule(lr){1-8}
		FedAvg & DNN && $0.02$  &$98.79   \pm 0.03$&& $0.03$  &$83.64 \pm 0.22 $ \\
		Per-FedAvg & DNN& & $0.02, 0.001$   & $98.90  \pm 0.02$& & $0.01, 0.001$ & $85.01   \pm 0.10$ \\ %85.09
		\OurAlg-GM & DNN& 30&$0.01$ & $99.16  \pm 0.03   $& 30 & $0.01$ & $84.17 \pm 0.35 $\\
		\OurAlg-PM & DNN&30 & $0.01$  & $\textbf{99.46}  \pm 0.01$& 30& $0.01$ & $\textbf{86.36} \pm 0.15$\\
		\cmidrule(lr){1-8}
%		FedAvg & MLR & & $0.02$  & $94.11\% $& & $0.02$  & $77.86\% $\\
%		Per-FedAvg & MLR& & $0.03, 0.003$   & $94.50\% $& & $0.03, 0.003$ & $79.91\% $\\
%		\OurAlg-GM & MLR& 15& $0.01$& $ 94.52 \% $ & 15 & $0.01$ & $79.28 \% $ \\
%		\OurAlg-PM & MLR& 15& $0.01$& \textbf{96.40\%}& 15 & $0.01$ & \textbf{82.55\%} \\
%		\cmidrule(lr){1-8}
%		FedAvg & DNN && $0.02$  &$98.74\% $&& $0.03$  &$83.32\% $ \\
%		Per-FedAvg & DNN& & $0.02, 0.001$   & $98.88\% $& & $0.01, 0.001$ & $84.76\% $ \\
%		\OurAlg-GM & DNN& 30&$0.01$ & $99.41 \%   $& 20 & $0.01$ & $84.44 \% $\\
%		\OurAlg-PM & DNN&30 & $0.01$  & \textbf{99.62\%} & 20& $0.01$ & \textbf{85.08\% } \\
%		\cmidrule(lr){1-8}
%	\begin{tabular}{lllll|lll}
%		\toprule
%		%\hline
%		\multirow{3}{*}{Algorithm} &
%		\multirow{3}{*}{Model} &
%		\multicolumn{6}{c}{Dataset} \\
%		\cmidrule{3-8}
%		& & \multicolumn{3}{c}{MNIST} & \multicolumn{3}{c}{Synthetic} \\
%		\cmidrule{3-8}
%		%\cline{3-8}
%		&  & $\lambda$ & $\eta$    & $Acc$ &$\lambda$ & $\eta$   & $Acc$ \\
%		\hline
%		FedAvg & MLR & & $0.02$  & $94.11\% $& & $0.02$  & $77.86\% $\\
%		Per-FedAvg & MLR& & $0.03(\hat{\alpha})$/$0.003(\hat{\beta})$   & $94.50\% $& & $0.03(\hat{\alpha})$/$0.003(\hat{\beta})$ & $79.91\% $\\
%		\OurAlg-GM & MLR& 15& $0.01$& $ 94.52 \% $ & 20 & $0.01$ & $79.28 \% $ \\
%		\OurAlg-PM & MLR& 15& $0.01$& \textbf{96.40\%}& 20 & $0.01$ & \textbf{82.55\%} \\
%		\hline
%		FedAvg & DNN && $0.02$  &$98.74\% $&& $0.03$  &$83.32\% $ \\
%		Per-FedAvg & DNN& & $0.02(\hat{\alpha})$/$0.001(\hat{\beta})$   & $98.88\% $& & $0.01$($\hat{\alpha}$)/$0.001$($\hat{\beta})$ & $84.76\% $ \\
%		\OurAlg-GM & DNN& 30&$0.01$ & $99.41 \%   $& 20 & $0.01$ & $84.44 \% $\\
%		\OurAlg-PM & DNN&30 & $0.01$  & \textbf{99.62\%} & 20& $0.01$ & \textbf{85.08\% } \\
%		\bottomrule
%		\cmidrule(r){1-6}
%		Algorithms & Dataset & Model & $\lambda$ & $\eta$   & $Acc$\\
%		\midrule
%		FedAvg  & MNIST& Logistic & $$ & $0.02$   & $94.11\% $\\
%		Per-FedAvg & MNIST& Logistic & $$ & $0.03(\hat{\alpha})$/$0.003(\hat{\beta})$   & $94.50\% $\\
%		\OurAlg-Global Model& MNIST & Logistic & $15$  &  $0.01$   & $ 94.52 \% $\\
%		\OurAlg-Personal Model & MNIST& Logistic& $15$ &  $0.01$  & $ 96.40 \% $\\
%		\midrule
%		FedAvg  & MNIST& DNN & $$ & $0.02$   & $98.74\% $\\
%		Per-FedAvg & MNIST& DNN & $$   & $0.02(\hat{\alpha})$/$0.001(\hat{\beta})$   & $98.88\% $\\
%		\OurAlg-Global Model & MNIST& DNN & $30$ &  $0.01$   &$99.41 \%   $\\
%		\OurAlg-Personal Model & MNIST& DNN& $30$  &  $0.01$  & $99.62 \%$\\
%		\bottomrule
	\end{tabular}
\end{table}
}

{From the experimental results, when the data among clients are non-i.i.d, both \OurAlg and Per-Avg gain higher testing accuracy than FedAvg as they allow the global model to be personalized for a specific client. However, by optimizing the personalized model approximately with multiple gradient updates and avoiding computing the Hessian matrix, the personalized model of \OurAlg is more advantageous than Per-FedAvg in terms of the convergence rate and the computation complexity.}

==> system_model.tex <==
We consider a system (or network) of one server and a set $\mathcal{N}$ of $N$ devices.
